A Deeper Look into Second-Order Feature Aggregation for LiDAR Place Recognition

Efficient LiDAR Place Recognition (LPR) compresses dense pointwise features into compact global descriptors. While first-order aggregators such as GeM and NetVLAD are widely used, they overlook inter-feature correlations that second-order aggregation naturally captures. Full covariance, a common second-order aggregator, is high in dimensionality; as a result, practitioners often insert a learned projection or employ random sketches -- both of which either sacrifice information or increase parameter count. However, no prior work has systematically investigated how first- and second-order aggregation perform under constrained feature and compute budgets. In this paper, we first demonstrate that second-order aggregation retains its superiority for LPR even when channels are pruned and backbone parameters are reduced. Building on this insight, we propose Channel Partition-based Second-order Local Feature Aggregation (CPS): a drop-in, partition-based second-order aggregation module that preserves all channels while producing an order-of-magnitude smaller descriptor. CPS matches or exceeds the performance of full covariance and outperforms random projection variants, delivering new state-of-the-art results with only four additional learnable parameters across four large-scale benchmarks: Oxford RobotCar, In-house, MulRan, and WildPlaces.

==> introduction.tex <==



\section{Introduction} 
\label{sec:intro}
LiDAR place recognition (LPR), the task of estimating previously visited places when traversing an environment, plays an important role for robotic and autonomous systems navigation, and Simultaneous Localisation and Mapping (SLAM)~\citep{cadena2016past,park2021elasticity}. 
LPR generally involves extracting features from LiDAR point clouds and comparing these features with those stored in a database for establishing correspondences with an appropriate similarity metric such as Euclidean distance. The aim is to recognize places even under continuous environmental conditions changes such as weather, lighting or viewpoint variations. 

\begin{figure}[h]
\centering
\includegraphics[width=0.5\linewidth]{chapters/top_plot.pdf}
\caption{Effectiveness of our \coolname{} over popular LPR pooling methods on Oxford RobotCar \citep{maddern20171}, \mulran{} (Sejong environment) \citep{kim2020mulran} and \wildplaces{} (Venman environment) \citep{knights2023wild} datasets. All methods used \minkloc{}~\citep{komorowski2022improving} features and evaluated on a single GPU. Compared in terms of Recall@1.}
\label{fig: top-page-fig}
\end{figure}

Feature pooling is mandatory in LPR methods as it combines and compresses the extracted local features from input point clouds with varying numbers of points to a fixed-size global descriptor per input pointcloud, reducing the dimensionality without sacrificing the relevant information for recognition. Traditional pooling methods used in LPR such as average pooling, max pooling,  GeM pooling \citep{radenovic2018fine} and NetVLAD pooling \citep{uy2018pointnetvlad} give computationally efficient yet effective mechanisms for reducing the dimension. These methods are also known as first-order pooling methods \citep{gao2016compact,lin2017improved} and they are limited in terms of their capacity to capture complex relationships in the features \citep{zhang2023kernel}. %
They dampen the most informative features, leading to a phenomenon known as ``feature burstiness", where discriminative details are diluted. These methods do not consider feature interactions, making them less effective in distinguishing between important details and irrelevant background noise, resulting in weaker performance.
In contrast, second-order pooling methods such as covariance pooling \citep{lin2017improved} capture complex feature relationships by going beyond first-order pooling, offering a much richer and discriminative representation suitable for robust LPR. They are less sensitive to the background (\eg{} points from the surface of roads in urban scenarios).
Despite their potential, these methods compute the full covariance matrix of features, which is high-dimensional and computationally burdensome, making them unsuitable for real-world robotic applications and large-scale environments. Furthermore, they significantly increase the database search time causing delays in LPR systems \citep{uy2018pointnetvlad}. How to effectively reduce the dimensionality of second-order pooling methods for LPR tasks is a relatively under-explored area in literature. 

To answer this question, we propose a \underline{C}ompact \underline{C}hannel \underline{C}orrelation \underline{R}epresentation (\coolname{}), that produces compact covariance matrices by leveraging the idea of channel partitioning. Specifically, instead of computing a full covariance matrix from the entire feature set as done in the existing methods, we partition the feature channels into smaller equal-sized groups, each forming smaller covariance matrices. These group-wise covariance matrices effectively capture local feature component correlations, which are then aggregated using a learnable weighted sum. This approach significantly reduces the dimensionality burden while keeping important information from each group, resulting representation that remains discriminative. Moreover, by focusing on smaller, manageable covariance matrices, \coolname{} enables faster database searches in large-scale LPR tasks. It keeps the advantage of second-order pooling -- capturing rich feature correlations, without the computational burdens typically associated with full covariance matrix computation.


In comparison with the pooling method of LoGG3D-net \citep{vidanapathirana2022logg3d}, which does not inherently produce a smaller covariance matrix but instead reduces the feature dimensions for obtaining smaller covariance matrices, our method produces a compact representation instead of a full covariance representation directly. In addition, we are scalable to large feature channels with a negligible computation cost. We are also significantly better than NetVLAD pooling \citep{uy2018pointnetvlad} popularly used in LPR in terms of both the size of learnable parameters and performance, as illustrated in Figure \ref{fig: top-page-fig} where we compare against other pooling methods. Furthermore, our proposed method is invariant to point permutations.

We conduct extensive experiments with our proposed method on four popular LPR datasets, namely, Oxford Robotcar \citep{maddern20171}, In-house \citep{uy2018pointnetvlad}, \mulran \citep{kim2020mulran} and \wildplaces \citep{knights2023wild}, to demonstrate its effectiveness. We also compare with the existing state-of-the-art, common first-order pooling methods used in LPR and two popular covariance pooling methods from the image domain \citep{gao2016compact,li2018towards}. 

